Modular Gene Dynamics and Network Theory at Mesoscopic Scale

Complex dynamical systems are often modeled as networks, with nodes representing dynamical units which interact through the network's links. Gene regulatory networks, responsible for the production of proteins inside a cell, are an example of system that can be described as a network of interacting genes. The behavior of a complex dynamical system is characterized by cooperativity of its units at various scales, leading to emergent dynamics which is related to the system's function. Among the key problems concerning complex systems is the issue of stability of their functioning, in relation to different internal and external interaction parameters. In this Thesis we study two-dimensional chaotic maps coupled through non-directed networks with different topologies. We use a non-symplectic coupling which involves a time delay in the interaction among the maps. We test the stability of network topologies through investigation of their collective motion, done by analyzing the departures from chaotic nature of the isolated units. The study is done on two network scales: (a) full-size networks (a computer generated scalefree tree and a tree with addition of cliques); (b) tree's characteristic sub-graph 4-star, as a tree's typical dynamical motif which captures its topology in smallest possible number of nodes and is suitable for time-delayed interaction. We study the dynamical relationship between these two network structures, examining the emergence of cooperativity on a large scale (trees) as a consequence of mesoscale dynamical patterns exhibited by the 4-star. (FULL ABSTRACT INSIDE THE TEXT)

==> letter-to-arxiv <==
Your submission cond-mat.levnajic.27653 was rejected.

      Your attempted submission to the archive has been rejected due to
the following unpacking errors:

 Problem unpacking references-thesis.bib: contained references-thesis.bib file, but no references-thesis.bbl file
  (include references-thesis.bbl, or submit without references-thesis.bib;
   and remember to verify references).

Contains:
 4star-coupling-picture1.eps: 52103 bytes
 4star-sna-with10iterations.eps: 153099 bytes
 MLE-averaged-initial-star-node1-09-positive.eps: 11460 bytes
 MLE-starnode1-048.eps: 8648 bytes
 MLE-starnode1-09.eps: 317067 bytes (looks big)
   %%Creator: GIMP PostScript file plugin V 1.17 by Peter Kirchgessner
 MLE-treenode745-09.eps: 249429 bytes
 SNA-starnode1-09-048-lypndistribution-mean=-00048.eps: 9175 bytes
 SNA-starnode1-09-048-lypndistribution.eps: 19619 bytes
 SNA-starnode1-09-048.eps: 139339 bytes
 S_n-pikovsky-inset.eps: 48093 bytes
 attr-0048-hub.eps: 83434 bytes
 attr-0048-node2.eps: 83950 bytes
 attractor-0048-formation-step1.eps: 147049 bytes
 attractor-0048-formation-step2.eps: 147498 bytes
 attractor-0048-formation-step3.eps: 147889 bytes
 attractor-0048-formation-step4.eps: 148724 bytes
 attractor-0048-formation-step5.eps: 150353 bytes
 attractor-0048-formation-step6.eps: 151177 bytes
 attractor-star-node1-y-signal.eps: 20591 bytes
 attractor-star-node1-y-signal_n.eps: 17967 bytes
 attractor-starnode1-09-048-lypndistribution.eps: 20490 bytes
 attractor-starnode1-09-048.eps: 122675 bytes
 bandwidth.eps: 859045 bytes (looks big)
   %%Creator: gnuplot 4.0 patchlevel 0
 bandwiths-histogram.eps: 22313 bytes
 bifur-evals-SNA-stable.eps: 16383 bytes
 bifur-evals-SNA-unstable.eps: 14731 bytes
 chaoticorbit-star-node0-y-signal.eps: 17886 bytes
 chaoticorbit-star-node0-y-signal_n.eps: 17726 bytes
 cliquenode-0049-y.eps: 18340 bytes
 cliquenode-0049.eps: 83618 bytes
 clusters-colorful.eps: 37859 bytes
 comparison-alltogether-rt-012.eps: 24547 bytes
 comparison-alltogether-rt-051.eps: 25494 bytes
 comparison-lypositive-nonperiodic-4star-1000ic.eps: 23071 bytes
 comparison-nonperiodic-allstruct-trans2x1e6.eps: 28042 bytes
 comparison-nonperiodic-mscnet-tree.eps: 20582 bytes
 comparison-nonperiodic-star-tree-regions.eps: 23526 bytes
 comparison-nonperiodic-star-tree.eps: 21703 bytes
 comparison-treenode745-MLE-nonperiodic-09.eps: 21279 bytes
 comparisonMLE-star-node1-node0-09-049.eps: 12362 bytes
 comparisonMLE-starnode1-treenode745-09-049.eps: 10198 bytes
 comparisonMLE-starnode1-treenode745-09.eps: 19308 bytes
 degreedist-comparison.eps: 20257 bytes
 diffusion.eps: 404612 bytes (looks big)
   %%Creator: gnuplot 4.0 patchlevel 0
 directed-allnodes-0022-example1.eps: 24057 bytes
 directed-allnodes-0022-example2.eps: 23767 bytes
 directed-allnodes-0022-example3.eps: 23973 bytes
 directed-lyp-00do08-5ic-allnodes-onehistogram.eps: 18195 bytes
 directeddynamics-motif-0022-pajek.eps: 87407 bytes
 directeddynamics-motif-005-pajek.eps: 92424 bytes
 distance-samecluster.eps: 17892 bytes
 dperiods_tree_avtraj008_comb.eps: 67084 bytes
 draft1.bbl: 24458 bytes
 draft1.tex: 285869 bytes
 ecoli-FTMLE-tf-and-nodes.eps: 421715 bytes (looks big)
   %%Creator: GIMP PostScript file plugin V 1.17 by Peter Kirchgessner
 ecoli-FTMLE-tf-sum-nodes.eps: 552157 bytes (looks big)
   %%Creator: GIMP PostScript file plugin V 1.17 by Peter Kirchgessner
 ecoli-connectedcomponent.eps: 299548 bytes
 ecoli-degreeranking-innout.eps: 28736 bytes
 ecoli-finalp-nodes-noise02.eps: 28838 bytes
 ecoli-full423-names.eps: 523088 bytes (looks big)
   %%Creator: GIMP PostScript file plugin V 1.17 by Peter Kirchgessner
 ecoli-noise-sigma-slope123.eps: 17106 bytes
 ecoli-p-flex-and.eps: 397060 bytes (looks big)
   %%Creator: GIMP PostScript file plugin V 1.17 by Peter Kirchgessner
 ecoli-p-flex-sum.eps: 438711 bytes (looks big)
   %%Creator: GIMP PostScript file plugin V 1.17 by Peter Kirchgessner
 ecoli-pajek-partition-tf-nodes.eps: 244956 bytes
 ecoli-relaxation-sum-and.eps: 26212 bytes
 ecoli-sigmap-nodes-and-noise001.eps: 381406 bytes (looks big)
   %%Creator: GIMP PostScript file plugin V 1.17 by Peter Kirchgessner
 ecoli-sigmap-nodes-sum-noise001.eps: 282129 bytes
 ecoli-slopes.eps: 179484 bytes
 ecoli-tf-nodeflex-and-19-89-122-135.eps: 21018 bytes
 ecoli-tf-nodeflex-sum-2-89-119-122.eps: 20452 bytes
 ecoli-trj-3tf-1ic.eps: 308132 bytes (looks big)
   %%Creator: gnuplot 4.2 patchlevel 0
 ecoli-trj-fixtf-3ic.eps: 394556 bytes (looks big)
   %%Creator: gnuplot 4.2 patchlevel 0
 ecoli-trj-fixtf-noise02-zoom.eps: 131651 bytes
 ecoli-trj-fixtf-noise02.eps: 168199 bytes
 ecoli-tt-relax-sum-and.eps: 17305 bytes
 finalstate-tree-012-allnodes-5militerations.eps: 70882 bytes
 gene-regulation-scheme.eps: 730572 bytes (looks big)
   %%Creator: CorelDRAW 12
 hopf-eigenvalues.eps: 16379 bytes
 hopf-phasespace-0014.eps: 86858 bytes
 initial-sync-09-021-truesftree-insetstar.eps: 4944088 bytes (looks big)
   %%Creator: GIMP PostScript file plugin V 1.17 by Peter Kirchgessner
 ly-0027-1e5iter-20000ic.eps: 24880 bytes
 ly-0054-1e5iter-20000ic.eps: 21498 bytes
 ly-048-1e5iter-20000ic.eps: 23038 bytes
 ly-048-1e5iter-zoomattractors.eps: 22253 bytes
 ly-4star-1e5iter-00-08-zoomattractor.eps: 422923 bytes (looks big)
   %%Creator: GIMP PostScript file plugin V 1.17 by Peter Kirchgessner
 ly-4star-1e5iter-00-08.eps: 287465 bytes
 ly-attr048-iter-hist.eps: 24154 bytes
 ly-qp0027-iter-hist+inset-ly-convtozero.eps: 35145 bytes
 ly-qp0027-iter-hist.eps: 25051 bytes
 ly-sna-iter-hist.eps: 25725 bytes
 lyabs-delta1e-4-4star-qporbits-1000ic.eps: 18718 bytes
 lyapunovdivergence.eps: 29988 bytes
 lyp-directed-0022-nodes-25ic.eps: 297028 bytes
 lyp-directed-005-nodes-25ic.eps: 308959 bytes (looks big)
   %%Creator: GIMP PostScript file plugin V 1.17 by Peter Kirchgessner
 lyp-directed-00do08-allnodes-5ic.eps: 728580 bytes (looks big)
   %%Creator: GIMP PostScript file plugin V 1.17 by Peter Kirchgessner
 lypnspectrums-starnode1-09-049.eps: 12419 bytes
 matrix-ecoli-connectedcomponent-network.eps: 990251 bytes (looks big)
   %%Creator: (ImageMagick)
 matrix-true-sf-1.eps: 330007 bytes (looks big)
   %%Creator: GIMP PostScript file plugin V 1.17 by Peter Kirchgessner
 max-distance-sna.eps: 23384 bytes
 minfree5maxfree10minclq4maxclq6-1010node-motifcolor.eps: 219975 bytes
 msct-tree-zerosteps.eps: 18568 bytes
 new-nonperiodic-456cliques.eps: 25641 bytes
 new-nonperiodic-comparison.eps: 20652 bytes
 new-periodization-comparison-averaged-012.eps: 40501 bytes
 new-periodization-comparison-examples.eps: 27498 bytes
 nodelayvsdelay-nonperiodic-new-star-125ic-trans5xe5-delta1e-8.eps: 20208 bytes
 nodelvsdel-nonperiodic-new-tree-1ic-trans5xe5-delta1e-8.eps: 20272 bytes
 nonperiodic-msct-allnodes-10ic.eps: 17383 bytes
 nonperiodic-new-328genenodes-directed-transe6-10ic+inset-pt.eps: 22345 bytes
 nonperiodic-new-328genenodes-transe6-1ic.eps: 18593 bytes
 nonperiodic-new-directed-transe6-nodebynode-20ic.eps: 305360 bytes (looks big)
   %%Creator: GIMP PostScript file plugin V 1.17 by Peter Kirchgessner
 nonperiodic-new-tree-5ic-delta1e-8-variouse.eps: 31911 bytes
 orbit-0022-example1.eps: 91540 bytes
 orbit-0022-example2.eps: 86586 bytes
 orbit-0022-example3.eps: 113743 bytes
 orbit-005-example1.eps: 91705 bytes
 orbit-005-example2.eps: 89650 bytes
 orbit-005-example3.eps: 90591 bytes
 orbitexample-attractor.eps: 431695 bytes (looks big)
   %%Creator: gnuplot 4.0 patchlevel 0
 orbitexample-chaos.eps: 294379 bytes
 orbitexample-regular.eps: 287384 bytes
 orbits-005-node119-3examples.eps: 168622 bytes
 orbits-005-node56-4examples.eps: 126691 bytes
 orbits-005-node86-3examples.eps: 174498 bytes
 parametersensitivity-4star-hubvsbranch-sna.eps: 186573 bytes
 partition-directed-nonperiodic-0022.eps: 282982 bytes
 partition-directed-nonperiodic-005.eps: 287095 bytes
 partition-pajek-motifsinecolinetwork.eps: 1181391 bytes (looks big)
   %%Creator: (ImageMagick)
 pd-eigenvalues.eps: 16377 bytes
 pd-phasespace-0015.eps: 13839 bytes
 periodization-pajek-0001-trans1e6.eps: 150926 bytes
 periodization-pajek-0001-trans2x1e5.eps: 160408 bytes
 periodization-pajek-0001-trans3x1e6.eps: 142823 bytes
 periodization-pajek-0001-trans4x1e5.eps: 157934 bytes
 periodization-tree.eps: 151150 bytes
 periods-dist-nodebynode-tree-012vs08.eps: 20094 bytes
 periods-statistics-240.eps: 19024 bytes
 periods-tree-hist-1ic-012.eps: 76400 bytes
 periods.eps: 16196 bytes
 periodsdist-msct-tree-clique6.eps: 22494 bytes
 prett_treechaosavtraj_MJU.eps: 31580 bytes
 qp-0027-freqspectrum.eps: 44420 bytes
 qp-0054-orbit-hub.eps: 88487 bytes
 qp-0054-orbit-node1.eps: 88403 bytes
 qp-0054-orbit-node2.eps: 53174 bytes
 ranking-periods-starnode1vstreenode745-09-0021-norepeat.eps: 22365 bytes
 ranking-periods-starnode1vstreenode745-09-008-norepeat.eps: 19692 bytes
 rankings-comparison.eps: 594637 bytes (looks big)
   %%Creator: gnuplot 4.0 patchlevel 0
 regularorbit-star-node0-y-signal.eps: 15899 bytes
 regularorbit-star-node0-y-signal_n.eps: 17956 bytes
 rettimes_phsp_SNA.eps: 27784 bytes
 rt-attractorSNA-048-qexpfit.eps: 43617 bytes
 rt-comparison-msct-tree-012.eps: 21134 bytes
 rt-comparison-msct-tree-051.eps: 22818 bytes
 rt-directed-0022-variousnodes.eps: 63765 bytes
 rt-directed-005-node119-4ic.eps: 99107 bytes
 rt-directed-005-node86-3ic.eps: 73206 bytes
 rt-directed-005-variousnodes.eps: 64468 bytes
 rt-starnode1-av-manyic.eps: 80977 bytes
 rt-starnode1-treezones-averaged.eps: 1139626 bytes (looks big)
   %%Creator: gnuplot 4.0 patchlevel 0
 rt-truesf-5ic-cha-attr.eps: 26558 bytes
 rt-truesf-5ic-qp-periodic.eps: 28761 bytes
 s040.eps: 533477 bytes (looks big)
   %%Creator: gnuplot 4.2 patchlevel 0
 s050.eps: 84527 bytes
 s090.eps: 102846 bytes
 sameclusternodes-partition-002.eps: 341323 bytes (looks big)
   %%Creator: GIMP PostScript file plugin V 1.17 by Peter Kirchgessner
 sigmaybar-directed-0022-pajek-partition.eps: 308755 bytes (looks big)
   %%Creator: GIMP PostScript file plugin V 1.17 by Peter Kirchgessner
 sigmaybar-directed-005-pajek-partition.eps: 303984 bytes (looks big)
   %%Creator: GIMP PostScript file plugin V 1.17 by Peter Kirchgessner
 single-gene-widder.eps: 9111 bytes
 sna-bifur.eps: 16380 bytes
 sna-hub.eps: 84516 bytes
 sna-node2.eps: 84917 bytes
 star-node1-comparison-nonperiodic-MLE.eps: 21278 bytes
 starbranch-0007-y.eps: 27210 bytes
 starbranch-0007.eps: 85502 bytes
 starbranch-0012-y.eps: 16855 bytes
 starbranch-0012.eps: 30062 bytes
 starbranch-0014-y.eps: 18397 bytes
 starbranch-0014.eps: 49056 bytes
 starbranch-0027-y.eps: 18281 bytes
 starbranch-0027.eps: 85554 bytes
 sync-treusf100-09-008-prag00001.eps: 509093 bytes (looks big)
   %%Creator: MATLAB, The Mathworks, Inc. Version 7.3.0.298 (R2006b). Operating System: SunOS 5.9 Generic_117171-09 sun4u.
 timeaverage-nodelay-star-node1-09.eps: 211341 bytes
 timeaverage-nodelay-treeallnodes-09.eps: 207778 bytes
 timeaverage-ybar-clique-09.eps: 237480 bytes
 timeaverage-ybar-msct-allnodes-09.eps: 204491 bytes
 timeaverage-ybar-starnode1-09.eps: 207610 bytes
 timeaverage-ybar-tree-allnodes-09.eps: 187525 bytes
 transient-times-comparison.eps: 16879 bytes
 transtime-statistics.eps: 16311 bytes
 tree-av-mu0012-0iterations.eps: 29987 bytes
 tree-av-mu0012-500000iterations.eps: 30016 bytes
 tree-av-mu0012-50000iterations.eps: 30016 bytes
 tree-clusterseparation-0012.eps: 32316 bytes
 tree-evals.eps: 26912 bytes
 tree-finalstate-5mil.eps: 245375 bytes
 tree-nonperiodic-node745.eps: 16996 bytes
 widder-scheme.eps: 323843 bytes (looks big)
   %%Creator: GIMP PostScript file plugin V 1.17 by Peter Kirchgessner
 ybar-directed-nodes-0022-500ic.eps: 243130 bytes
 ybar-directed-nodes-005-307ic.eps: 229114 bytes
 ybar-directed-transe6-1ic.eps: 274279 bytes
 ybar-msct.eps: 12408 bytes
 ybar-sigma-tree-dispersion-large.eps: 62445 bytes
 ybar-sigma-tree-dispersion-small.eps: 57639 bytes
 ybar-star-allnodes-250ic-00-08.eps: 237832 bytes
 ybar-tree-allnodes-012.eps: 26218 bytes

Warnings:

Author 1: Zoran Levnaji\'c

 Title field appeared capitalized, formerly:
  Title: MODULAR GENE DYNAMICS AND NETWORK THEORY AT MESOSCOPIC SCALE
 levnajic-thesis-arxiv.tar: unpacked 207 files from tar file
 REMOVED references-thesis.bib
 We don't run bibtex in the auto-TeXing procedure. If you use it, include
 in your submission the .bbl file which bibtex produces on your home machine;
 otherwise your references will not come out correctly. We don't run bibtex
 because the .bib database files can be quite large, and the only thing
 necessary to make the references for a given paper is the .bbl file.


END

